Keeping Your Eye on the Ball: Trajectory Attention in Video Transformers

In video transformers, the time dimension is often treated in the same way as the two spatial dimensions. However, in a scene where objects or the camera may move, a physical point imaged at one location in frame $t$ may be entirely unrelated to what is found at that location in frame $t+k$. These temporal correspondences should be modeled to facilitate learning about dynamic scenes. To this end, we propose a new drop-in block for video transformers -- trajectory attention -- that aggregates information along implicitly determined motion paths. We additionally propose a new method to address the quadratic dependence of computation and memory on the input size, which is particularly important for high resolution or long videos. While these ideas are useful in a range of settings, we apply them to the specific task of video action recognition with a transformer model and obtain state-of-the-art results on the Kinetics, Something--Something V2, and Epic-Kitchens datasets. Code and models are available at: https://github.com/facebookresearch/Motionformer

==> figs/distillation_ablation.tex <==

\begin{table*}[tb]
\footnotesize
\caption{\textbf{Comparison experiments and ablations.} We compare key parameters and settings of our proposed method. We report results model performance at epoch 100 and with 30 frames and without transformer unless noted otherwise.
}\label{tab:ablation}
	\begin{subtable}[b]{.33\linewidth}\centering
		{\includegraphics[width=0.99\linewidth]{figs/alpha_ablation.pdf}}	
	\end{subtable}
	\begin{subtable}[b]{.33\linewidth}\centering
		{\includegraphics[width=0.99\linewidth]{figs/num_frames_ablation.pdf}}	
	\end{subtable}
	\begin{subtable}[b]{.33\linewidth}\centering
		{\includegraphics[width=0.99\linewidth]{figs/distill_layer_ablation.pdf}}	
	\end{subtable}
	\\
	\vspace{4em}
\vspace{-2.0em}
\end{table*}

==> figs/motion_transformer.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.99\linewidth]{figs/motionformer.png}
\vspace{-1em}
\end{center}
   \caption{\textbf{Motioformer Arhcitecture.} 
  We break our input into patches....
   \label{fig:splash}
   }
\end{figure}


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> scratch.tex <==
% \subsection{Background}\label{s:background}
\subsection{Video transformers overview}\label{s:overview}
% Notation
% Jabri et al. 2020:
% Video is often treated as a simple extension of an image into time, modeled as a spatio-temporal XY T volume [72, 118, 14]. Yet, treating time as yet another dimension is limiting [26]. One practical issue is the sampling rate mismatch between X and Y vs. T. But a more fundamental problem is that a physical point depicted at position (x, y) in frame t might not have any relation to what we find at that same (x, y) in frame t + k, as the object or the camera will have moved in arbitrary (albeit smooth) ways. This is why the notion of temporal correspondence — “what went where" [113] — is so fundamental for learning about objects in dynamic scenes, and how they inevitably change.

\paragraph{Input:}
The input to a video transformer is a video clip $\bX \in \reals^{T_0 \times H_0 \times W_0 \times C}$ with $T_0$ frames of height $H_0$, width $W_0$ and $C=3$ RGB channels. We consider two methods for mapping a video into a sequence of tokens $\bZ^0 \in \reals^{T \times H \times W \times D}$.
% Image patches vs video tubelets:
[Explain non-overlapping image patches vs tubelets]
% Input embedding:
[Explain input embedding]
% Positional encoding:
[Explain positional encoding]
\Ishan{It maybe useful to introduce `tokens' here and then distinguish the different forms of attention in terms of what token relationships they capture.}

The core of a transformer network is the attention operation that shares information between the tokens. Previous work \cite{bertasius2021spacetime, arnab2021vivit} has explored several ways to adapt the attention mechanism to video data. The two popular approaches are joint space-time attention and divided space-time attention~\cite{neimark2021video,bertasius2021spacetime,arnab2021vivit}.
%
For self-attention, the queries $\bQ$, keys $\bK$ and values $\bV$ are computed as linear projections of the input $\bZ$, such that $\bQ = \bZ \bW_q$, $\bK = \bZ \bW_k$, and $\bV = \bZ \bW_v$, for projection matrices $\bW_i \in \reals^{D \times D}$.
\newpage


\paragraph{Joint space-time attention:} [Explain using Fig 2]
\Ishan{Need an easier way to contrast this equation from divided-space time.}
This operation computes bidirectional dot-product attention, treating tokens equally across space and time. It is given by
\begin{align}
    \attn(\bQ, \bK, \bV) &= \softmax\left( \bQ \bK\transpose / \sqrt{D} \right) \bV,
\end{align}
where $\bQ, \bK, \bV, \in \reals^{ST \times D}$ are the queries, keys and values, and the softmax operation, $\softmax$, is taken over the last dimension.

\paragraph{Divided space-time attention:} [Explain using Fig 2]
This attention block alternates between computing self-attention spatially (across all tokens extracted from the same temporal index) and temporally (across all tokens extracted from the same spatial index). That is, it alternates between
\begin{align}
%    \attn(\bQ_t, \bK_t, \bV_t) &= \softmax\left( \bQ_t \bK_t\transpose / \sqrt{D} \right) \bV_t \text{, and}\\
%    \attn(\bQ_s, \bK_s, \bV_s) &= \softmax\left( \bQ_s \bK_s\transpose / \sqrt{D} \right) \bV_s,
%    A_\mathrm{space} = \left[\attn(\bQ_{s,:,:}, \bK_{s,:,:}, \bV_{s,:,:})\right]_{s=1}^S,\qquad
%    A_\mathrm{time} = \left[\attn(\bQ_{:,t,:}, \bK_{:,t,:}, \bV_{:,t,:})\right]_{t=1}^T,\qquad
    A_\mathrm{space} = \left[\attn(\bQ_s, \bK_s, \bV_s)\right]_{s=1}^S,\qquad
    A_\mathrm{time} = \left[\attn(\bQ_t, \bK_t, \bV_t)\right]_{t=1}^T,\qquad
    A = A_\mathrm{space} \odot A_\mathrm{time}
\end{align}
for all temporal indices $t \in [1, T]$ and all spatial indices $s \in [1, S]$, where $\bQ_t, \bK_t, \bV_t \in \reals^{S \times D}$ and $\bQ_s, \bK_s, \bV_s \in \reals^{T \times D}$ are the temporally and spatially indexed queries, keys, and values, and the softmax operation is taken over the last dimension.
To index the matrices, we reshape $\reals^{ST \times D} \to \reals^{S \times T \times D}$ and index the temporal or spatial dimension.
The resulting matrices are then concatenated across the dimension reduced by the attention, yielding two same-sized tensors $A_\mathrm{space}$ and $A_\mathrm{time}$, which are element-wise multiplied.

% An alternative late fusion approach is given as
% \paragraph{Factorised encoder attention:} % ViViT

These approaches to the fundamental component of the transformer network---the self-attention block---do not encode an appropriate inductive bias for video data. Instead, they treat features identically across space and time or restrict temporal information transfer to axis-aligned paths. \Ishan{This needs to be explained better. Right now it isn't clear why the divided space time attention cannot capture paths.}
We propose an alternative self-attention block, inspired by optical flow networks, where features are pooled along motion paths.
%a better inductive bias
% smooth variation of features along motion paths

\subsection{Trajectory attention}\label{s:attention}

% What we're actually doing is closer to divided space-time than joint space-time. We do the spatial-only part, and the time-only part, it's just that the time-only part uses inter-frame correlations to compute the features. The reason it looks like joint space-time is because those inter-frame correlations can be computed more efficiently that way, but conceptually it's different.
\Ishan{Would be clearer if explained in terms of tokens right here, without equations.}
To encourage the network to pool information along motion paths, we form an all-pairs correlation volume between and within frames. This is identical to the correlation volume extracted by an optical flow network, modulo a linear projection, applied to image patches rather than pixels. This is used to pool features within a frame from those locations where objects in the query patch may have moved. These motion-warped features are then pooled temporally using the standard attention operation.
% The encoder for an optical flow network typically forms a correlation volume.

Given a set of input tokens $\bZ^{l} \in \reals^{ST \times D}$, the queries, keys, and values are obtained via linear projections $\bQ^{l} = \bZ^{l} \bW_q^{l}$, $\bK^{l} = \bZ^{l} \bW_k^{l}$, and $\bV^{l} = \bZ^{l} \bW_v^{l}$, for projection matrices $\bW_i^{l} \in \reals^{D \times D}$.
Then for all temporal indices $t \in [1, T]$, we compute
\begin{align}
    \bY_t^{l} &= \attn(\bQ^{l}, \bK_t^{l}, \bV_t^{l}) = \softmax \left( \bQ^{l} {\bK_t^{l}}\transpose / \sqrt{D} \right) \bV_t^{l} \label{eq:spatial_attention}
\end{align}
where $\bY_t^{l}, \bQ^{l} \in \reals^{ST \times D}$, and $\bK_t^{l}, \bV_t^{l} \in \reals^{S \times D}$.
%where the softmax operation is taken over the last dimension.
This can be expressed as
\begin{align}
    \bY_t^{l} &= \bD_t^{-1} \bA_t \bV_t^{l}, \hspace{12pt} \bA_t = \exp(\bQ^{l} {\bK_t^{l}}\transpose / \sqrt{D}), \hspace{12pt} \bD_t = \diag(\bA_t \ones_S),
\end{align}
where $\ones_S$ is the ones vector of length $S$.
The outputs are stacked to give $\bY^{l} = [\bY_1^{l}, \ldots, \bY_T^{l}] \in \reals^{ST \times T \times D}$, and are interpreted as motion-warped features: each query token is associated with one feature per frame that pools information from features along the query's putative motion path(s).

% Temporal attention:
Now that we have a 1D sequence of features for each query token, we need to pool information across the temporal dimension. While average pooling is a reasonable choice, it cannot take into account the differing temporal distances between frames. We might expect some drop-off in the reliability of information contained in temporally distant frames. Consequently, we use 1D temporal attention to reason about which features to strengthen and which to attenuate. 
%
There is an immediate design choice between using the original queries or a linear projection of $\bY$. The latter has the benefit of having aggregated information across the spatial dimension, which has recently been shown to help resolve correspondence ambiguities in the context of optical flow estimation \cite{jiang2021learning}. We demonstrate empirically that this also provides value for video classification tasks.
Conceptually, using queries where the information has been pooled across spatial dimensions brings our method into alignment with divided space-time attention, separating the spatial and temporal pooling operations. The key difference however is that the temporal information is pooled across motion-warped features, rather than axially. These motion-warped features are computed efficiently in \eqnref{eq:spatial_attention} as the output of inter-frame spatial attention.

% Projection:
We again take linear projections
$\tilde{\bQ}^{l} = \diag_T(\bY^{l}) \tilde{\bW}_q^{l} \in \reals^{ST \times D}$,
$\tilde{\bK}^{l} = \bY^{l} \tilde{\bW}_k^{l} \in \reals^{ST \times T \times D}$, and
$\tilde{\bV}^{l} = \bY^{l} \tilde{\bW}_v^{l} \in \reals^{ST \times T \times D}$,
where $\diag_T(\cdot)$ denotes taking the diagonal elements of the two time dimensions.
That is, a query for frame $i$ should only aggregate information from frame $i$.
%
Then for all space-time indices $i \in [1, ST]$, we compute
\begin{align}
    \tilde{\bY}_i^{l} &= \attn(\bQ_i^{l}, \bK_i^{l}, \bV_i^{l}) = \softmax \left( \bQ_i^{l} {\bK_i^{l}}\transpose / \sqrt{D} \right) \bV_i^{l}
\end{align}
and stack the output $\tilde{\bY}^{l} = [\tilde{\bY}_1^{l}, \ldots, \tilde{\bY}_{ST}^{l}] \in \reals^{ST \times D}$.
This corresponds to standard attention with a batch dimension of size $ST$.

% Remainder of the pipeline:
The remainder of the layer follows the standard transformer pipeline with a feed-forward network (MLP) and a residual connection, generating the layer output $\bZ^{l+1} = \text{MLP}(\tilde{\bY}^l) + \bZ^{l}$.

% % MHA: Move to implementation details
% In practice, we use multi-head attention.


% \paragraph{Learned approximation.}

% \Eqnref{eq:prob-attn-conditional} implies that $A$ and $q$ are independent given $U$ ($A \indep q \mid U$), which is not necessarily true. To learn this parametric model from data, we would like to ensure that the approximation of \eqnref{eq:prob-attn-conditional} follows closely the full attention (\eqnref{eq:prob-attn}). We thus propose to minimise the KL divergence between them. Since computing the full attention every iteration would obviously negate the computational benefits of the approximation, we compute only a \emph{stochastic estimate} of it, by subsampling the columns, \ie, only computing it for a subset of the outputs:
% \begin{equation}
% \min_{p}KL(\tilde{P}(A \mid p) \| P(A))=\min_{p}\mathbb{E}_{j\sim\textrm{categorical}(n)}KL(\tilde{P}(A_{:j} \mid p) \| P(A_{:j})),\label{eq:prob-attn-objective}
% \end{equation}
% \begin{equation}
% \min_{p}KL(P(A) \| \tilde{P}(A \mid p))=\min_{p}\mathbb{E}_{i\sim\textrm{categorical}(m)}KL(P(A_{i:}) \| \tilde{P}(A_{i:} \mid p)),\label{eq:prob-attn-objective}
% \end{equation}
% where the dependence of the approximation on the prototypes $p$ is made explicit. \Eqnref{eq:prob-attn-objective} (right hand side) is an unbiased estimator for the true KL-divergence (left hand side), though at the expense of higher variance (due to sampling). As such, the overall computational cost scales as $\cO(m+n)$.

% An alternative objective is the mutual information between $A$ and $U$, given by
% \begin{equation}
% I(A, U) = \expectation_{U} \left[ \kl \left( P(A \mid U) \| P(A) \right) \right],
% \label{eq:prob-attn-objective2}
% \end{equation}
% which can be computed using
% \begin{equation}
% I(A_{:j}, U_{:j}) = \sum_\ell P(U_{lj}) \kl_i \left( P(A_{:j} \mid U_{\ell j}) \| P(A_{:j}) \right)
% = \sum_\ell \softmax(p\transpose k)_{\ell j} \kl_i \left( \softmax(q\transpose p)_{:\ell} \| \softmax(q\transpose k)_{:j} \right).
% \label{eq:prob-attn-objective3}
% \end{equation}
% Again, a stochastic estimate is obtained by subsampling the rows:
% \begin{equation}
% \min_{p} I(A, U(p)) = \min_{p}\mathbb{E}_{i\sim\textrm{categorical}(m)} I(A_{i:}, U(p)).
% \label{eq:prob-attn-objective4}
% \end{equation}

% Variants: temporal averaging (instead of temporal attention), approximation

%For the true softmax distribution $X = \softmax(QK\transpose)$ and the approximated distribution $Y = \softmax (QL\transpose) \softmax(LK\transpose)$, with softmax taken over the last dimension,
%\begin{align}
%    \cL_\text{KL} &= \kl(X \| Y) = \sum_{ij} X_{ij} \ln \frac{X_{ij}}{Y_{ij}}\\
%    \pp{\cL_\text{KL}}{L} &= -\sum_{ij} \frac{X_{ij}}{Y_{ij}} \pp{Y_{ij}}{L} = 0\\
%    \pp{Y_{ij}}{L} &= A_{ij} (Q_i + K_j) - A_{ij} \ones_d\transpose \odot \softmax(LK\transpose) K - \ones_l\transpose A_{ij} \softmax(Q_i L\transpose)\transpose Q_i\\
%    A_{ij} &= \softmax(Q_i L\transpose)\transpose \odot \softmax(L K_j\transpose) \in \reals^{\ell \times 1}\\
%    Y_{ij} &= \sum_k A_{ijk} \in \reals
%\end{align}
%Does this lead to a closed-form for $L$ or any condition on it?
%Note that $\softmax(L K_j\transpose) = \softmax(L K\transpose)_{:,j}$ in this notation.

% \begin{align}
%     \kl(X \| Y) &= \sum_{ij} X_{ij} \ln \frac{X_{ij}}{Y_{ij}}\\
%     &= \sum_{ij} \softmax_j (Q_i K_j\transpose) \ln \frac{\softmax_j (Q_i K_j\transpose)}{\softmax (Q_i L\transpose)\softmax_j (L K_j\transpose)}\\
%     &= \sum_{ij} \softmax_j (Q_i K_j\transpose) \ln \frac{\exp(Q_i K_j\transpose)}{\sum_j \exp(Q_i K_j\transpose)} \frac{\sum_k \exp(Q_i L_k\transpose) \sum_j \exp(L K_j\transpose)}{\sum_k \exp(Q_i L_k\transpose) \exp(L_k K_j\transpose)}
% \end{align}
% not quite...

==> tabs/abl_shuffled.tex <==
\begin{table}
\begin{center}

\begin{tabular}{ccc}
\toprule
Model &  Shuffled   & Acc. \\
\midrule
VideoTransformer & {\color{gray}\xmark} & $XX$ \\
MotionFormer  & {\color{gray}\xmark} & $XX$ \\
\hline
VideoTransformer   & \cmark & $XX$ \\
MotionFormer  & \cmark & $XX$\\

\bottomrule
\end{tabular} 
\end{center} 
\vspace{0.5em}
\caption{\textbf{Impact of Shuffled Frames.} We show that the Motionformer is much sensitive to motion transformations such as shuffling and reveral, while the VideoTransformer is invariant to these changes.\label{tab:ablation:shuffled}}
% \vspace{-1em}
\end{table}

==> tabs/abl_softmax.tex <==
\begin{tabular}{l c c c}
	\toprule
	Trajectory  & Flops. & K-400 & SSv2  \\
	\midrule
	Joint Softmax & 369.5  & XX & XX    \\ 
	Frame Softmax  &  369.5  & \bf 79.7 & \bf 66.5    \\ 
	 \bottomrule
\end{tabular}
